First release of Apertif imaging survey data

(Abridged) Apertif is a phased-array feed system for WSRT, providing forty instantaneous beams over 300 MHz of bandwidth. A dedicated survey program started on 1 July 2019, with the last observations taken on 28 February 2022. We describe the release of data products from the first year of survey operations, through 30 June 2020. We focus on defining quality control metrics for the processed data products. The Apertif imaging pipeline, Apercal, automatically produces non-primary beam corrected continuum images, polarization images and cubes, and uncleaned spectral line and dirty beam cubes for each beam of an Apertif imaging observation. For this release, processed data products are considered on a beam-by-beam basis within an observation. We validate the continuum images by using metrics that identify deviations from Gaussian noise in the residual images. If the continuum image passes validation, we release all processed data products for a given beam. We apply further validation to the polarization and line data products. We release all raw observational data from the first year of survey observations, for a total of 221 observations of 160 independent target fields, covering approximately one thousand square degrees of sky. Images and cubes are released on a per beam basis, and 3374 beams are released. The median noise in the continuum images is 41.4 uJy/bm, with a slightly lower median noise of 36.9 uJy/bm in the Stokes V polarization image. The median angular resolution is 11.6"/sin(Dec). The median noise for all line cubes, with a spectral resolution of 36.6 kHz, is 1.6 mJy/bm, corresponding to a 3-sigma HI column density sensitivity of 1.8 x 10^20 atoms cm^-2 over 20 km/s (for a median angular resolution of 24" x 15"). We also provide primary beam images for each individual Apertif compound beam. The data are made accessible using a Virtual Observatory interface.

==> incl-acks.tex <==
EAKA is supported by the WISE research programme, which is financed by the Dutch Research Council (NWO)KMH acknowledges financial support from the State Agency for Research of the Spanish Ministry of Science, Innovation and Universities through the "Center of Excellence Severo Ochoa" awarded to the Instituto de Astrofísica de Andalucía (SEV-2017-0709), from the coordination of the participation in SKA-SPAIN, funded by the Ministry of Science and Innovation (MCIN). KMH acknowledges funding from the Europeaní Research Council under the European Union’s Seventh Framework Programme (FP/2007-2013)/ERC Grant Agreement No. 291531 (‘HIStoryNU’).JMvdH acknowledges funding from the Europeaní Research Council under the European Union’s Seventh Framework Programme (FP/2007-2013)/ERC Grant Agreement No. 291531 (‘HIStoryNU’).OMB acknowledges funding from the Dutch Research Council (NWO) under the Vici research program 'ARGO' with project number 639.043.815YM acknowledges funding from the European Research Council under the European Union's Seventh Framework Programme (FP/2007-2013)/ERC Grant Agreement No. 617199.
LCO acknowledges funding from the European Research Council under the European Union's Seventh Framework Programme (FP/2007-2013)/ERC Grant Agreement No. 617199.
IPM acknowledges funding from the Netherlands Research School for Astronomy (grant no. NOVA5-NW3-10.3.5.14).AAP acknowledges support of the STFC consolidated grant ST/S000488/1. RS acknowledges funding from the European Research Council under the European Union's Seventh Framework Programme (FP/2007-2013)/ERC Grant Agreement No. 617199.
JvL acknowledges funding from the European Research Council under the European Union’s Seventh Framework Programme (FP/2007-2013) / ERC Grant Agreement n. 617199 (`ALERT'), and from Vici research programme `ARGO' with project number 639.043.815, financed by the Dutch Research Council (NWO).DV acknowledges support from the Netherlands eScience Center (NLeSC) under grant ASDI.15.406

==> incl-authors.tex <==
%% -- Your edits may get overwritten by the formatting script -- check with JVL -- 

%% ----------------- Authors ---------------
%% -- One-liner for submission form, etc. --
%% E. A. K. Adams, B. Adebahr, W. J. G. de Blok, H. Dénes, K. M. Hess, A. Kutkin, D. M. Lucero, Raffaella Morganti, V. A. Moss, T. A. Oosterloo, E. Orr\'u, R. Schulz, J. M. van der Hulst, O. M. Boersma, M. Bouwhuis, L.  Connor, A. H. W. M. Coolen, S. Damstra, R. de Goei, T.J. Dijkema, N. Ebbendorf, Y.G. Grange, A.W. Gunst, H.A. Holties, B. Hut, M.V. Ivashina, G.I.G. J\'ozsa, G. Marcel Loose, Yogesh Maan, M. Mancini, A'. Mika, H. Mulder, M. J. Norden, A. R. Offringa, L. C. Oostrum, I. Pastor-Marazuela, D.J. Pisano, A.A. Ponomareva, J.W. Romein, M Ruiter, A.P. Schoenmakers, J.J. Sluman, R. Smits, K.J.C Stuurwold, A. S. van Amesfoort, W.A. van Cappellen, R. van den Brink, D. van der Schuur, G. N. J. van Diepen, Joeri van Leeuwen, Joris Verstappen, N.P.E Vilchez, Dany Vohl, K.J. Wierenga, S. J. Wijnholds, E.E.M. Woestenburg, A.W. Zanting, J. Ziemke 
%% -- Latex formatted ------------------- --
   E.~A.~K.~Adams       \inst{\ref{astron} \and \ref{kapteyn}}

\and B.~Adebahr           \inst{\ref{airub}}

\and W.~J.~G.~de~Blok     \inst{\ref{astron} \and \ref{cpt} \and \ref{kapteyn}}

\and H.~Dénes            \inst{\ref{astron}}

\and K.~M.~Hess           \inst{\ref{iaa} \and \ref{astron} \and \ref{kapteyn}}

\and A.~Kutkin            \inst{\ref{astron} \and \ref{lebedev}}

\and D.~M.~Lucero         \inst{\ref{virginiatech}}

\and Raffaella~Morganti   \inst{\ref{astron} \and \ref{kapteyn}}

\and V.~A.~Moss           \inst{\ref{csiro} \and \ref{sydney} \and \ref{astron}}

\and T.~A.~Oosterloo      \inst{\ref{astron} \and \ref{kapteyn}}

\and E.~Orr\'u            \inst{\ref{astron}}

\and R.~Schulz            \inst{\ref{astron}}

\and J.~M.~van~der~Hulst  \inst{\ref{kapteyn}}

\and O.~M.~Boersma        \inst{\ref{uva}}

\and M.~Bouwhuis          \inst{\ref{nikhef}}

\and L.~~Connor           \inst{\ref{uva} \and \ref{caltech}}

\and A.~H.~W.~M.~Coolen   \inst{\ref{astron}}

\and S.~Damstra           \inst{\ref{astron}}

\and R.~de~Goei           \inst{\ref{astron}}

\and T.J.~Dijkema         \inst{\ref{astron}}

\and N.~Ebbendorf         \inst{\ref{astron}}

\and Y.G.~Grange          \inst{\ref{astron}}

\and A.W.~Gunst           \inst{\ref{astron}}

\and H.A.~Holties         \inst{\ref{astron}}

\and B.~Hut               \inst{\ref{astron}}

\and M.V.~Ivashina        \inst{\ref{chalmers}}

\and G.I.G.~J\'ozsa       \inst{\ref{mpifr} \and \ref{rhodes}}

\and G.~Marcel~Loose      \inst{\ref{astron}}

\and Yogesh~Maan          \inst{\ref{ncra} \and \ref{astron}}

\and M.~Mancini           \inst{\ref{astron}}

\and A'.~Mika             \inst{\ref{astron}}

\and H.~Mulder            \inst{\ref{astron}}

\and M.~J.~Norden         \inst{\ref{astron}}

\and A.~R.~Offringa       \inst{\ref{astron} \and \ref{kapteyn}}

\and L.~C.~Oostrum        \inst{\ref{astron} \and \ref{uva} \and \ref{escience}}

\and I.~Pastor-Marazuela  \inst{\ref{uva} \and \ref{astron}}

\and D.J.~Pisano          \inst{\ref{wvu} \and \ref{gwac} \and \ref{cpt}}

\and A.A.~Ponomareva      \inst{\ref{oxford}}

\and J.W.~Romein          \inst{\ref{astron}}

\and M~Ruiter             \inst{\ref{astron}}

\and A.P.~Schoenmakers    \inst{\ref{astron}}

\and J.J.~Sluman          \inst{\ref{astron}}

\and R.~Smits             \inst{\ref{astron}}

\and K.J.C~Stuurwold      \inst{\ref{astron}}

\and A.~S.~van~Amesfoort  \inst{\ref{astron}}

\and W.A.~van~Cappellen   \inst{\ref{astron}}

\and R.~van~den~Brink     \inst{\ref{astron} \and \ref{tricas}}

\and D.~van~der~Schuur    \inst{\ref{astron}}

\and G.~N.~J.~van~Diepen  \inst{\ref{astron}}

\and Joeri~van~Leeuwen    \inst{\ref{astron} \and \ref{uva}}

\and Joris~Verstappen     \inst{\ref{kapteyn} \and \ref{astron}}

\and N.P.E~Vilchez        \inst{\ref{}}

\and Dany~Vohl            \inst{\ref{uva} \and \ref{astron}}

\and K.J.~Wierenga        \inst{\ref{}}

\and S.~J.~Wijnholds      \inst{\ref{astron}}

\and E.E.M.~Woestenburg   \inst{\ref{astron}}

\and A.W.~Zanting         \inst{\ref{astron}}

\and J.~Ziemke            \inst{\ref{astron} \and \ref{oslocit}}

} 

%% ----------------- Institutes --------------- 
\institute{ASTRON, the Netherlands Institute for Radio Astronomy, Oude Hoogeveensedijk 4,7991 PD Dwingeloo, The Netherlands\label{astron}
  \and
Kapteyn Astronomical Institute, PO Box 800, 9700 AV Groningen, The Netherlands\label{kapteyn}
  \and
Astronomisches Institut der Ruhr-Universit{\a}t Bochum (AIRUB), Universit{\a}tsstrasse 150, 44780 Bochum, Germany\label{airub}
  \and
Dept.\ of Astronomy, Univ.\ of Cape Town, Private Bag X3, Rondebosch 7701, South Africa\label{cpt}
  \and
Instituto de Astrof\'{i}sica de Andaluc\'{i}a (CSIC), Glorieta de la Astronom\'{i}a s/n, 18008 Granada, Spain\label{iaa}
  \and
Astro Space Center of Lebedev Physical Institute, Profsoyuznaya Str. 84/32, 117997 Moscow, Russia\label{lebedev}
  \and
Department of Physics, Virginia Polytechnic Institute and State University, 50 West Campus Drive, Blacksburg, VA 24061, USA\label{virginiatech}
  \and
CSIRO Astronomy and Space Science, Australia Telescope National Facility, PO Box 76, Epping NSW 1710, Australia\label{csiro}
  \and
Sydney Institute for Astronomy, School of Physics, University of Sydney, Sydney, New South Wales 2006, Australia\label{sydney}
  \and
Anton Pannekoek Institute, University of Amsterdam, Postbus 94249, 1090 GE Amsterdam, The Netherlands\label{uva}
  \and
NIKHEF, National Institute for Subatomic Physics, Science Park 105, 1098 XG Amsterdam, Netherlands\label{nikhef}
  \and
Cahill Center for Astronomy, California Institute of Technology, Pasadena, CA, USA\label{caltech}
  \and
Dept.\ of Electrical Engineering, Chalmers University of Technology, Gothenburg, Sweden\label{chalmers}
  \and
Max-Planck-Institut f\ur Radioastronomie, Auf dem H\ugel 69, D-53121 Bonn, Germany\label{mpifr}
  \and
Department of Physics and Electronics, Rhodes University, P.O. Box 94, Makhanda, 6140, South Africa\label{rhodes}
  \and
National Centre for Radio Astrophysics, Tata Institute of Fundamental Research, Pune 411007, Maharashtra, India\label{ncra}
  \and
Netherlands eScience Center, Science Park 140, 1098 XG, Amsterdam, The Netherlands\label{escience}
  \and
Department of Physics and Astronomy, West Virginia University, White Hall, P.O. Box 6315, Morgantown, WV 26506, USA\label{wvu}
  \and
Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505\label{gwac}
  \and
Oxford Astrophysics, Denys Wilkinson Building, University of Oxford, Keble Rd, Oxford, OX1 3RH, UK\label{oxford}
  \and
Tricas Industrial Design \& Engineering, Zwolle, The Netherlands\label{tricas}
  \and
University of Oslo Center for Information Technology, P.O. Box 1059, 0316 Oslo, Norway\label{oslocit}}
